Multiple gaps and some finitizations of club and CH

We continue the development of the theory of capturing schemes over $\omega_1$ by analyzing the relation between the capturing construction schemes (whose existence is implied by Jensen's $\Diamond$-principle) and both the Continuum Hypothesis and Ostaszewski's $\clubsuit$-principle. Formally, we show that the property of being capturing can be viewed as the conjunction of two properties, one of which is implied by $\clubsuit$ and the other one by CH. We apply these principles to construct multiple gaps, entangled sets and metric spaces without uncountable monotone subspaces.

==> gaps.tex <==


\section{Almost distoint families and multiple gaps}\label{sectiongaps}

Motivated by Amir's result (\cite{Amir}) stating that the space $l_\infty/c_0$ is not injective, Avil\'es and Todor\v{c}ev\'ic introduced in \cite{multiplegaps} the concept of an $n$-gap as a natural generalization of the well-studied notion of gaps as presented by Hausdorff in the early 1900's. In there, they showed that unlike usual gaps, Hausdorff's result about the existence of $(\omega_1,\omega_1)$-gaps in $ZFC$ can not be extended to greater dimensions without assuming extra axioms. Precisely, they showed that under $MA_\theta(\sigma-k\text{-linked})$ there are no $n$-gaps formed by $\theta$-generated ideals in $\mathscr{P}(X)$ for $n>k$ and $X$ countable. Particularly, this means that the non-existence of $\omega_1$-$n$-gaps (see Definition \ref{typegapdef} below) is consistent with the usual axioms of set theory for each $n\geq 3$.  On the other hand, they proved that $CH$ implies the existence  of such $n$-gaps for every $n$. The theory  has been further developed in papers such as \cite{analyticstrongngaps}, \cite{finitebasismultiplegaps} and \cite{isolatingsubgaps}, with a particular emphasis on the study of  multiple gaps formed by analytic families. However, beyond the results mentioned above, not as much is known about multiple gaps in the context of $\omega_1$.

In this section we will show that under $CA^\Delta_n$ and $\text{CA}^\rho_n$, the theory of $n$-gaps generated by sets of size $\omega_1$ is as rich as it could be (Theorem \ref{allgapsthm}). 
In order to do so,  we will construct an almost disjoint family of size $\omega_1$ with very strong properties. We will then use its elements as building blocks for a large variety of objects associated to $n$-gaps.

Let $X$ be a countable set and $\mathcal{T}\subseteq[X]^\omega$. We say that $\mathcal{T}$ is a \textit{tower}\footnote{It is also common in the literature to call these objects pre-towers, and towers are pre-towers which are maximal with respect to the end-extension. As we won't be dealing with maximal pre-towers, we've opted to simply refer to them as "towers" to simplify the notation.} if it is well-ordered with respect to $\subseteq^*$. Furthermore, for an ordinal $\kappa$, we say that $\mathcal{T}$ is a $\kappa$-tower whenever it is a tower and $ot(\mathcal{T})=\kappa.$


\begin{definition}[$n$-gaps and $n$-pregaps]
Let $X$ be a countable set, $n\in \omega$ and $\mathcal{L}_0,\dots,\mathcal{L}_{n-1}\subseteq\mathscr{P}(X)$. We say that $(\mathcal{L}_i\,:\,i<n)$ is an $n$-\emph{pregap} if $\mathcal{L}_i$  is orthogonal to $\mathcal{L}_j$ for all $i\not=j$. A function  $c:n\longrightarrow \mathscr{P}(X)$ is said to \emph{separate} $(\mathcal{L}_i\,:\, i<n)$ if $L\subseteq^*c(i)$ and $C\cap R=^*\emptyset$ for each $i<n$ and $L\in\mathcal{L}_i$. We say that $(\mathcal{L}_i\,:\,i<n)$ is an $n$-\textit{gap} if it is an $n$-pregap and there is no function $c$ separating it.
\end{definition}
For $n=2$, we will say that a set $C\subseteq X$ \emph{separates} a pregap $(\mathcal{L},\mathcal{R})$ if $L\subseteq^*C$ and $R\cap C=^*\emptyset$ for all $L\in \mathcal{L}$ and $R\in\mathcal{R}$. It should be clear that such set exists if and only if there a function $c$ separating $(\mathcal{L},\mathcal{R})$. Particularly, this means that the notion of a $2$-pregap and $2$-gap coincides with the standard notions of pregap and gap respectively.
\begin{definition}[Type of an $n$-gap]\label{typegapdef} Let $2\leq n\in \omega$, and $\langle (X_i,\leq_i)\rangle_{i<n}$ be a family of partial orders. We say that an $n$-pregap $(\mathcal{L}_i\,:\,i<n)$ is an \emph{$(X_i\,:\,i<n)$-pregap} (or \emph{$(X_i\,:\,i<n)$-n-pregap)} if $(\mathcal{L}_i,\subseteq^*)$ is isomorphic to $(X_i,\leq_i)$ for each $i<n$. Furthermore, if $(\mathcal{L}_i\,:\,i<n)$ is an $n$-gap we will refer to it as an \emph{$(X_i\,:\,i<n)$-gap} (or \emph{$(X_i\,:\,i<n)$-n-gap}) and if $(X_i,\leq_i)=(X,<)$ for all $i<n$, we will simply refer to the gap as an $X$-$n$-gap.
\end{definition}

\begin{definition} Let $\mathcal{A}$ be an almost disjoint family of size $\omega_1$ over a set $X$. We say that $\mathcal{A}$ is:
\begin{itemize}
    \item $n$-\emph{inseparable} if for any  pairwise disjoint $\mathcal{L}_0,\dots,\mathcal{L}_{n-1}\in [\mathcal{A}]^{\omega_1}$, the tuple $(\mathcal{L}_i\,:\,i<n)$ forms an $n$-gap. We suppress the index if $n=2$.
    \item  \emph{Jones} if for any two disjoint  $\mathcal{L}\in [\mathcal{A}]^{\omega}$ and $\mathcal{R}\in [\mathcal{A}]^{\omega_1}$,  $(\mathcal{L},\mathcal{R})$ is not a gap. 
  \end{itemize}
\end{definition}
   The first construction of an inseparable family was done in \cite{luzin1947subsets} by Nikol\'ai Nikol\'ayevich Luzin. A Jones family was implicitly constructed by F. B. Jones in \cite{jones1937concerning}. Although, at first glance,  inseparable and Jones seem to be incompatible properties, a construction of a inseparable-Jones family was obtained in \cite{guzman2019mathbb} by the Guzm\'an
, Hru\v{s}\'ak and Koszmider (building from work by Koszmider in \cite{onconstructionswith2cardinals}). We would like to point out that the highly complex construction of the mentioned family is carried out through the use of simplified morasses. In 
the next theorem we show that the existence of an $n$-inseparable-Jones family follows from the existence of both an $n$-$\rho$-capturing and an $n$-$\Delta$-capturing scheme. As these types of schemes exist without assuming any extra axioms in the particular case where $n=2$, this also yields an elementary construction of an inseparable-Jones family from $ZFC$ alone.

\begin{theorem}\label{luzinjonestheorem}Let $\mathcal{F}$ be a scheme of type $\langle m_k,n_k,r_k\rangle_{k\in \omega}$. Given $k\in \omega$, consider $N_k= m_{k-1}^{n_k}\times \{k\}$ and $N=\bigcup\limits_{k\in \omega} N_k$. Given $\alpha\in \omega_1$ and $k\in \omega$ we define $$A^k_\alpha:=\{\sigma\in N_k\,:\,\Xi_\alpha(k)\geq 0\text{ and }\sigma(\Xi_\alpha(k))=\lVert \alpha\rVert_{k-1}\}$$
and $A_\alpha:=\bigcup\limits_{k\in \omega} A_k$.  Then $\mathcal{A}_\mathcal{F}=\langle A_\alpha\rangle_{\alpha\in \omega_1}$ is a Luzin-Jones $AD$-family. Furthermore, if  either $\mathcal{F}$ is $n$-$\rho$-capturing or $n$-$\Delta$-capturing, then $\mathcal{A}_\mathcal{F}$ is an $n$-inseparable.
\begin{proof}Each $A_\alpha$ is infinite because $\Xi_\alpha(k)\geq 0$ for infinitely many $k$'s. It is also easy to see that for distinct $\alpha$ and $\beta$ we have that\begin{equation}
    A_\alpha\cap A_\beta\subseteq \bigcup\limits_{k\leq \rho(\alpha,\beta)} (A_\alpha^k\cap A_\beta^k).
\end{equation}
Therefore, $A_\mathcal{F}$ is an AD family. Before proving the second part note that if $D\in[\omega_1]^n$ and $k\in \omega$ are such that $\Xi_{D(i)}(k)=i$ for each $i$, then \begin{equation}
   \{\sigma\in N_k\,:\,\forall i<n\,( \sigma(i)=\lVert D(i)\rVert_{k})\}\subseteq \bigcap\limits_{i<n} A^k_{D(i)}.
\end{equation}
So in particular, $\big(\bigcap\limits_{i<n} A^k_{D(i)}\big)\cap N_k\not=\emptyset$.\\
Assume that $\mathcal{F}$ is  $n$-$\rho$-capturing (resp. $n$-$\rho$-capturing) and let $\langle I_i\rangle_{i<n}$ be a sequence of uncountable disjoint subsets of $\omega_1$. We shall prove that $( \langle A_\alpha\rangle_{\alpha\in I_i}\,:\,i<n)$ is an $n$-gap. Assume towards a contradiction that 
this is not the case and let $c:n\longrightarrow \mathscr{P}(N)$ be a witness of this fact. By refining each $I_i$, we may assume without loss of generality that for each $i<n$ there is $k_i\in \omega$ so that $A_\alpha^k\subseteq c(i)$ for all $\alpha\in I_i$. As $\bigcap\limits_{i<n} c(i)$ is finite, there is $k>\max(k_i\,:i<n)$ for which this intersection is disjoint from $A_l$ for each $l\geq k$. Now, we construct a family $\mathcal{D}\subseteq[\omega_1]^n$ be an uncountable family of pairwise disjoint sets so that $D(i)\in I_i$ for all $D\in \mathcal{D}$ and $i<n$. Siince $\mathcal{F}$ is $n$-$\rho$ -capturing (resp. $n$-$\Delta$-capturing) there exists a subfamily $\langle D_i\rangle_{i<n}$ of $\mathcal{D}$ and $l>k$ for which $\langle D_i\rangle_{i<n}$ is $\rho$-captured (resp.$\Delta$-captured) at level $l$. Since the $D_i$'s are pairwise disjoint, we have that $\Xi_{D_i(i)}(l)=i$ for each  $i<n$. Therefore, $\emptyset\not=\big(\bigcap\limits_{i<n}A^k_{D_i(i)} \big)\cap N_l\subseteq \big(\bigcap\limits_{i<n} c(i)\big)\cap N_l$. This is a contradiction so we are done.

We will end the proof by showing that $\mathcal{A}$ is a Jones family. For this purpose define  $C_\beta$ as $$\bigcup\limits_{k\in\omega}\big(\bigcup\limits_{\alpha\in (\beta)_k } A^{k+1}_\alpha\big)$$ for each $\beta\in\omega_1$. We will show that $C_\beta$ separates $(\langle A_\alpha\rangle_{\alpha\leq \beta},\langle A_\alpha\rangle_{\delta> \beta})$. Indeed, if $\alpha\leq\beta$ then $A^{k+1}_\alpha\subseteq C_\beta$ for 
each $k\geq \rho(\alpha,\beta)$, so in particular $A_\alpha\subseteq^*C_\beta$. On the other hand, if $\delta>\beta$ then $A^{k+1}_\delta\cap A^{k+1}_\alpha=\emptyset$ for any $k\geq \rho(\delta,\beta)$ and each $\alpha\in (\beta)_k$. This is because for any such $\alpha$ we have that $\rho(\alpha,\delta)\leq k$. Consequently $A_\delta\cap C_\beta=^*\emptyset$.
\end{proof}
    
\end{theorem}
The previous construction yields an almost disjoint family which satisfies a lot more properties than just being $n$-inseparable and Jones. For the rest this section we will analyze those properties. The following definitions are essential for that task.


Let $(X,\leq)$ be a partial order. We say that $x\in X$ is \textit{succesor-like} if $pred(x)$ is finite and cofinal in $(-\infty,x)$.



\begin{definition}[Almost disjoint representation]\label{Luzinrepdef} Let $(X,\leq)$ be a partial order of size $\omega_1$. An \textit{almost disjoint representation of $X$} (Shortly, $AD$-representation) is an ordered pair $(\mathcal{T},\mathcal{A})$ consisting of two families of infinite subsets of $\omega$ indexed as $\langle T_x\rangle_{x\in X}$ and $\langle A_x\rangle_{x\in X}$ respectively. Furthermore, $\mathcal{A}$ is an $AD$ family and for all $x,y\in X$ the following properties hold:
\begin{enumerate}[label=$(\alph*)$]
\item $A_x\subseteq T_x.$

\item If $y\not\leq x$, then $A_y\subseteq^*T_y\backslash T_x$.
\item If $\inf(x,y)$ exists, then $T_x\cap T_y=^*T_{\inf(x,y)}.$

\item If $x$ is succesor-like, then $$T_x\backslash\big(\bigcup\limits_{z\in pred(x)}T_z\big)=^*A_x.$$
\item If $x$ and $y$ are incompatible, then $T_x\cap T_y=^*\emptyset.$


\end{enumerate}
In particular $(\mathcal{T},\subseteq^*)$ is order isomorphic to $X$ by virtue of the points $(b)$ and $(c)$. In the case there is $(\mathcal{T},\mathcal{A})$ a Luzin representation of $X$ we say that $\mathcal{A}$ \textit{codes} $X$.
\end{definition}

Let us say that a partial order $(X,\leq)$ is $\omega_1$-like if it is well-founded, $|X|=\omega_1$ and $|(-\infty,x)|\leq \omega$ for all $x\in X$.


\begin{proposition}\label{propositionwellfounded}Let $(Y,\leq)$ be a partial order of cardinality $\omega_1$. There is a well-founded cofinal $X\subseteq Y$ with $|(-\infty, x)_X|\leq \omega$ for each $x\in X$.
\begin{proof} Enumerate $Y$ as $\langle y_\alpha\rangle_{\alpha\in \omega_1}$.  Define $X$ as the set of all $y_\beta$'s such that $y_\beta\not\leq y_\alpha$ for each $\alpha<\beta$. Of course $X$ is well-founded as for each $x,z\in X$ with $x=y_\alpha$ and $z=y_\beta$ it happens that if $x<z$ then $\alpha<\beta$. Because of this we also have that $(-\infty,\, y_\beta)_X\subseteq \{y_\alpha\,:\,\alpha<\beta\}$ for each $y_\beta\in X$. Lastly $X$ is cofinal in $Y$ because for each $\beta\in \omega_1$ the element $y_{\xi_\beta}\in X$ where  $\xi_\beta=\min(\,\alpha\leq \beta\,:\, y_\alpha \geq y_\beta\,)$.
\end{proof}
\end{proposition}
The following lemma is easy.
\begin{lemma}\label{bijectionlemma}Let $(X,\leq)$ be $\omega_1$-like. Then there is a bijection $\phi:X\longrightarrow \omega_1$ with $\phi(x)<\phi(y)$ for all $x<y\in X.$
\end{lemma}

Let $(X,\leq)$ $\omega_1$-like and $\phi:X\longrightarrow \omega_1$ as above. In the following lemma, in some sense, we will pull back a construction scheme from $\omega_1$ to some sort of \say{construction scheme} on $X$. This suggests that the theory of construction schemes could be generalized to other partial orders of size $\omega_1$. The extend and utility of this idea remains mainly unexplored.

\begin{lemma}\label{Mklemma}Let $\mathcal{F}$ be a scheme and let $X$ and $\phi$ be as in Lemma \ref{bijectionlemma}. For each $x\in X$ and $k\in\omega$ define $M^k_x=\{\, z\leq x\,:\, \phi(z)\in (\phi(x))_k\,\}$. The following properties hold for each $x,y\in X$ and $k\in\omega$:
\begin{enumerate}[label=$(\arabic*)$]
\item  If $\inf(x,y)$ exists and $k>\rho^{\phi[\{x,y,\inf(x,y)\}]}$, then $M^k_x\cap M^k_y=M^k_{\inf(x,y)}.$
\item[$(\frac{3}{2})$] If $y\leq x$ and $k>\rho^{\phi[\{x,y\}]}$, then $M^k_y\subseteq M^k_x$.
\item If $y\not\leq x$, then $y\in M^k_y\backslash M^k_x.$
\item If $x$ is succesor-like and $k>\rho^{\phi[pred(x)\cup\{x\}]}$, then $M^k_x\backslash\big( \bigcup\limits_{z\in pred(x)} M^k_z \big)=\{x\}$.
\item If $x$ and $y$ are incompatible,  then $M^k_x\cap M^k_y=\emptyset.$
\end{enumerate}
\begin{proof}
The points (2) and (4) are trivial and the point ($\frac{3}{2}$) follows directly from (1). Therefore,  we will only prove (1) and (3).

\begin{claimproof}[Proof of  $(1)$] Since $\phi$ preserves the order then $\phi(\inf(x,y))\leq \min(\phi(x),\phi(y))$ which implies that $(\phi(\inf(x,y))_k\sqsubseteq (\phi(x))_k\cap (\phi(y))_k$. In this way, if $z\in M^k_{\inf(x,y)}$ then $z\leq x,y$ by definition of the infimum, and $z$ belongs to both $(\phi(x))_k$ and $(\phi(y))_k$ because $z\in (\phi(\inf(x,y)))_k$. Therefore $z\in M^k_x\cap M^k_y$. On the other hand, if $z\in M^k_x\cap M^k_y$ then $z\leq x$ and $z\leq y$, so $z\leq \inf(x,y)$. Furthermore, $\phi(z)\in (\phi(x))_k\cap (\phi(y))_k$ and $\phi(z)\leq \phi(\inf(x,y))$. As $(\phi(\inf(x,y)))_k$ is an initial segment of such intersection then $\phi(z)$ belongs to it. Consequently $z\in M^k_{\inf(x,y)}$. 
\end{claimproof}
\begin{claimproof}[Proof of $(3)$] Note that since $x\not\leq z$ for any $z\in pred(x)$ then $x\in M^k_x\backslash M^k_z$ for any such $z$. This proves the inclusion from right to left. To show that the one from left to right also holds, let $$w\in M^k_x\backslash\big( \bigcup\limits_{z\in pred(x)} M^k_z \big).$$
Suppose towards a contradiction that $w<x$ and consider $z\in pred(x)$ with $w\leq z$. Since $k>\rho(\phi(x),\phi(z))$ we conclude that $(\phi(z))_k\sqsubseteq (\phi(x))_k$. But then  $\phi(w)\in (\phi(z))_k$ because $\phi(w)\leq \phi(z)$ and $\phi(w)\in (\phi(x))_k$. Consequently $w\in M^k_z$ which is a contradiction. This finishes the proof.
  \end{claimproof}  

\end{proof}
\end{lemma}
In the next theorem we show that not only a great variety of partial orders posses an $AD$ representation, but that the family  $\mathcal{A}_\mathcal{F}$ constructed in the Theorem \ref{luzinjonestheorem} codes all of them. For that reason it will be convenient to recall some basic facts regarding such family.


We have a countable set $N$ and $\langle N_k\rangle_{k\in\omega}$ a partition of $N$ into finite sets. For each $\alpha\in \omega_1$ we have $A_\alpha^k\subseteq N_k$ and we defined $A_\alpha=\bigcup\limits_{k\in \omega} A^{k+1}_\alpha$ and $\mathcal{A}_\mathcal{F}=\langle A_\alpha\rangle_{\alpha\in \omega_1}$. One key feature of $\mathcal{A}$ is that: \begin{center}If $\alpha,\beta\in\omega_1$ are distinct and $k>\rho(\alpha,\beta)$ then $A^k_\alpha\cap A^k_\beta=\emptyset.$
\end{center}

    


\begin{theorem}\label{luzinreptheorem}Let $\mathcal{A}_\mathcal{F}$ be the $AD$ family constructed in Theorem \ref{luzinjonestheorem} and let $(X,\leq)$ an $\omega_1$-like order. Then there is a family $\mathcal{T}=\langle T_x\rangle_{x\in X}\subseteq [\omega]^{\omega}$ and a re-indexing of $\mathcal{A}$ as $\langle\hat{A}_x\rangle_{x\in X}$ so that $(\mathcal{T},\mathcal{A})$ is an almost disjoint representation of $X$.
\begin{proof}Let $\phi:X\longrightarrow \omega_1$ be as in Lemma \ref{bijectionlemma} and
$ M^k_x$ be as in Lemma 
\ref{Mklemma} for any $x\in X$ and $k\in \omega$. Fix $x\in X$ and let $\hat{A}_x=A_{\phi(x)}.$
This defines the re-indexing of $\mathcal{A}$. Now, for each $k\in\omega$ and $x\in X$, let 
$$T^k_x=\bigcup \{\,A_{\phi(z)}^{k+1}\,:\,z\in M^k_x\,\}=\bigcup\{\,A^{k+1}_\xi\,:\,\xi\in \phi[M^k_x]\,\}$$
$$T_x=\bigcup\limits_{k\in\omega}T^k_x.$$
We claim that $(\mathcal{T},\mathcal{A})$ is an almost disjoint representation of $X$. In the following paragraphs we will show that the points $(a)$, $(b)$, $(c)$, $(d)$ and $(e)$ of Definition \ref{Luzinrepdef} are satisfied for such pair. 
\begin{claimproof}[Proof of $(a)$]Given $k>0$ we have that $A^k_{\phi(x)}\subseteq T^{k-1}_x$ because $x$ is always an element of $M^k_x$. Therefore $\hat{A}_x=A_{\phi(x)}\subseteq T_x$.   
\end{claimproof}
 Before proving the remaining points let us fix some notation. Given $P\in[\omega_1]^{<\omega}$ and $k\in\omega$, let $A^k_P=\bigcup\{A^k_\alpha\,:\,\alpha\in P\}$. Note that if $P,Q\in [\omega_1]^{<\omega}$ and $k>\rho^{P\cup Q}$ then, by virtue of the key feature of $\mathcal{A}$ highlighted just before this theorem, we have the following:

 $$A^k_P\cap A^k_Q=A^k_{P\cap Q},$$
$$A^k_P\cup A^k_Q=A^k_{P\cup Q},$$
$$A^k_{P}\backslash A^k_Q=A^k_{P\backslash Q}.$$

We will apply these three equalities for finite sets of the form $\phi[M^k_x]$. More precisely, observe that if $x,y\in X$ and $k>\rho(\phi(x),\phi(y))$ then $\rho^{\phi[M^k_x]\cup \phi[M^k_y]}<k+1$. This is because if we take  $F\in \mathcal{F}_k$ with $\phi(x),\phi(y)\in F$, then $\phi[M^k_x]\cup \phi[M^k_y]=\phi[M^k_x\cup M^k_y]\subseteq (\phi(x))_k\cup (\phi(y))_k\subseteq F.$ 

\begin{claimproof}[Proof of $(c)$]Let $x,y\in X$ and suppose that $\inf(x,y)$ exists.  Take an arbitrary $k>\rho^{\phi[\{x,y,\inf(x,y)\}]}$. By means of the point $(1)$ of Lemma  \ref{Mklemma}, $M^k_x\cap M^k_y=M^k_{\inf(x,y)}$. In this way: \begin{align*}
T^k_x\cap T^k_y =A^{k+1}_{M^k_x}\cap A^{k+1}_{M^k_y}
=A^{k+1}_{M^k_x\cap M^k_y}
=A^{k+1}_{M^k_{\inf(x,y)}}=T^k_{\inf(x,y)}.
\end{align*}
Therefore, $T_x\cap T_y=\bigcup\limits_{k\in\omega} \big( T^k_x\cap T^k_y\big)=^*\bigcup \{T^k_{\inf(x,y)}\,:\, k>\rho^{\phi[x,y,\inf(x,y)]}\}=^*T_{\inf(x,y)}.$
\end{claimproof}
The remaining parts of the theorem are proved in a completely similar way. Because of this, we leave the calculations to the reader. 
\end{proof}
\end{theorem}
The following result greatly extends Hausdorff's theorem about the existence of an $(\omega_1,\omega_1)$-gap.

\begin{theorem}[Under $CA^\Delta_n$ or $\text{CA}^\rho_n$] \label{allgapsthm}
Let  $\langle (X_i,<_i)\rangle_{i<n}$ is a family of partial orders of cofinality $\omega_1$. Then there are cofinal $X'_i\subseteq X_i$ for each $i$, so that there is an $(X'_i\,:\,i<n)$-gap.
\begin{proof}
 Without loss of generality we may assume that $X_i\cap X_j=\emptyset$ for any two distinct $i$ and $j$. By applying Proposition \ref{propositionwellfounded} we get, for each $i$, an $\omega_1$-like  $X'_i\subseteq X_i$ an cofinal subsets of $X_i$. Let $Z=\bigcup\limits_{i<n}X'_i$ 
and $<_Z:=\big(\bigcup\limits_{i<n} <_i\big)\cap Z^2$ . That is, $x<_Z y$ if and only if therer is $i$ for which $x,y\in X'_i$ and $x<_{X_i} y$. It is straightforward that $(Z,<_Z)$ is an $\omega_1$-like order. 
Furthermore, if $x\in X'_i$ and $y\in X_j'$  for $i\not=j$, then there is no $z\in Z$ with $z\leq_Z x, y.$ In virtue of Theorem \ref{luzinreptheorem}, there is a Luzin representation of $Z$, namely $(\mathcal{T},\mathcal{A})$. Due to  Definition \ref{Luzinrepdef} it follows that $(\langle T_x\rangle_{x\in X'_i}\,:\,i<n)$  is an $(X'_i\,:\,i<n)$-pregap.
We claim that this is in fact a gap. For this just note that any function $c$ separating $(\langle T_x\rangle_{x\in X'_i}\,:\,i<n)$ would also separate $(\langle A_x\rangle_{x\in X'_i}\,:\,i<n)$ by the point (a) of Definition \ref{Luzinrepdef}. But this is impossible since $\mathcal{A}$ is $n$-inseparable and each $X'_i$ is uncountable.
\end{proof}
\end{theorem}
\subsection{The gap cohomology group} In order to illustrate the power of the almost disjoint family constructed above, we now extend the work done by Daniel Talayco in \cite{cohomologytalayco}. Specifically, we will study the size of groups defined in a similar context as Talayco and prove that, under certain assumptions, these groups are as big as possible.
\begin{definition}[$*$-lower semi-lattice]Let $X$ be an infinite set.
We say that a family $\mathcal{T}\subseteq [X]^{\omega}$ is a \textit{$*$-lower semi-lattice} if  for any $A,B\in \mathcal{T}$ there is $C\in \mathcal{T}$ so that $A\cap B=^*C.$ In other words, $\{[A]\,:\,A\in \mathcal{T}\}$ is a lower semi-lattice in $\mathscr{P}(X)/\text{FIN}$.
\end{definition}
\begin{remark}Towers are particular cases of $*$-lower semi-lattices.
\end{remark}
\begin{definition}[Coherent Subsystems]\label{cohsystemsdef} Let $\mathcal{T}$ be a $*$-lower semi-lattice over a countable set $X$. A function $g:\mathcal{T}\longrightarrow \mathscr{P}(X)$ is said to be a \textit{coherent subsystem of $\mathcal{T}$} if for any $A,B\in \mathcal{T}$, the following happens:
\begin{enumerate}[label=$(\arabic*)$]
\item $g(A)\subseteq A$,
\item if $B\subseteq^* A$ then $g(A)\cap B=^*g(B)$.
\end{enumerate}
 We say that $g$ is \textit{trivial} if there is $C\in \mathscr{P}(X)$ so that $C\cap A=^*g(A)$ for any $A\in \mathcal{T}$. In this case, we say that $C$ \textit{trivializes} $g$. The set of all coherent subsystems of $\mathcal{T}$ is denoted as $C(\mathcal{T})$ and the set of all trivial coherent subsystem is denoted as $Tr(\mathcal{T}).$
\end{definition}
\begin{definition}Let $\mathcal{T}$ be a $*$-lower semilattice over a countable set $X$ and $g$ be a coherent subsystem of $\mathcal{T}$. We denote the sequence $(g(A),A\backslash g(A))_{A\in\mathcal{T}}$ as $\mathcal{C}(\mathcal{T},g).$
    
\end{definition}
The following lemma is easy. We prove it just to emphasise the reason of defining coherent subsystems just for $*$-lower semi-lattices.
\begin{lemma}\label{lemmacoherentsubsystempregap}Let $\mathcal{T}$ be a $*$-lower semi-lattice and let $g$ be a coherent subsystem of $\mathcal{T}$. Then $\mathcal{C}(\mathcal{T},g)$ is a pregap. Furthermore, $g$ is non-trivial if and only if $\mathcal{C}(\mathcal{T},g)$ forms a gap.

\begin{proof}Let $A,B\in \mathcal{T}$. We need to prove that $g(A)\cap (B\backslash g(B))=^*\emptyset.$ For this let $C\in \mathcal{T}$ be so that $C=^*A\cap B$. Then \begin{align*}g(A)\cap B=^* (g(A)\cap A)\cap B=^*g(A)\cap C
=^*g(C)=^*g(B)\cap C\subseteq ^*g(B).
\end{align*}
This finishes the argument. Now we will prove the proposed equivalence.
\begin{claimproof}[Proof of $\Rightarrow$] We will prove this by contra-positive. Suppose that there is a set $C$ separating the pregap $\mathcal{C}(\mathcal{T},g)$. For any $A\in \mathcal{T}$ we have that $g(A)\subseteq^* C$ and $C\cap (A\backslash g(A))=^*\emptyset.$ In this way, $C\cap A=^*g(A)$. We conclude that $C$ trivializes $g$. 
\end{claimproof}
\begin{claimproof}[Proof of $\Leftarrow$] Again, by contra-positive. Suppose that there is $C$ which trivializes $g$. Then $C\cap A=^*g(A)$ for any $A\in \mathcal{T}$. In particular $g(A)\subseteq^* C$ and $C\cap (A\backslash g(A))=\emptyset$. We conclude that $C$ separates $\mathcal{C}(\mathcal{T},g)$.
\
\end{claimproof}
\end{proof}
\end{lemma}


\begin{definition}Let $\mathcal{T}$ be a $*$-lower semi-lattice over a set $X$. For $f,g\in C(\mathcal{T})$ we can define $f\cdot g\in C(\mathcal{T})$ given as: $$(f\cdot g)(A)= f(A)\Delta g(A).$$
\end{definition}
The following lemma is easy.
\begin{lemma}
$C(\mathcal{T})$ is an abelian (Boolean)\footnote{A group $(G,\cdot, e)$ is Boolean if $g\cdot g=e$ for any $g\in G$. Equivalently, $G$ is a vector space over $\mathbb{Z}_2$. In particular, the isomorphism type of $G$ is completely determined by its cardinality.} group with respect to this operation and $Tr(\mathcal{T})$ is a subgroup of it. 
\end{lemma}
Since $C(\mathcal{T})$ is abelian, then $Tr(\mathcal{T})$ is a normal subgroup. Therefore, we can consider the quotient induced by it.
\begin{definition}[Gap cohomology group] We define the \textit{gap cohomology group of $\mathcal{T}$} as the quotient of these two groups. That is,  $$G(\mathcal{T})=C(\mathcal{T})/Tr(\mathcal{T}).$$
We  say that $f,g\in C(\mathcal{T})$ are \textit{cohomologous} if the class of $f$ is equal to the class of $g$ inside $G(\mathcal{T})$, or equivalently, if $f\cdot g\in Tr(\mathcal{T})$. 
\end{definition}
\begin{rem}If $\mathcal{T}$ has size $\omega_1$, then $|G(\mathcal{T})|\leq 2^{\omega_1}.$
    
\end{rem}
In \cite{cohomologytalayco}, Daniel E. Talayco defined the gap cohomology group for the particular case of $\omega_1$-towers. In there he showed that the $2^\omega\leq |G(\mathcal{T})|$ for any $\omega_1$-tower $\mathcal{T}$. In order to do that, he proved the following Theorem.
\begin{theorem}[The $\aleph_0$ gap theorem] let $\mathcal{T}=\langle T_\alpha\rangle_{\alpha\in \omega_1}$ be an $\omega_1$-tower. There is  a sequence of functions $\langle f_\alpha\rangle_{\alpha\in\omega_1}$ with the following properties:
\begin{itemize}
\item $\forall \alpha\in \omega_1\,(\,f_\alpha:T_\alpha\longrightarrow \omega\,)$,
\item $\forall \alpha<\beta\in \omega_1\, (\,f_\alpha|_{T_\alpha\cap T_\beta}=^*f_\beta|_{T_\alpha\cap T_\beta}\,),$
\item $\forall m<n\in\omega\,(\, (f_\alpha^{-1}[\{m\}],f_{\alpha}^{-1}[\{n\}]\,)_{\alpha\in\omega_1}\textit{ is a Hausdorff gap }).$ 

\end{itemize}
\end{theorem}
He also proved that the $\Diamond$-principle implies that the size of this group is always $2^{\omega_1}$. Later, Stevo Todor\v{c}evi\'{c} noted that the $\aleph_0$ gap theorem already gives you the previous conclusion without assuming any extra axioms (see Theorem 32 in \cite{cohomologytalaycotrees}). Namely, if $2^{\omega}=2^{\omega_1}$ the result is clear due to Talayco's calculations. On the other hand, if $2^{\omega}<2^{\omega_1}$ then the result follows from an easy counting argument involving the quotient structure of $G(\mathcal{T}).$
In \cite{Agapcohomologygroup}, Charles Morgan constructed an $\omega_1$-tower whose gap cohomology group can be explicitly calculated. This construction was carried through the use of morasses. Finally, in \cite{coherentfamilyoffunctions}, Ilijas Farah improved the $\aleph_0$ gap theorem. This was achieved by considering the following concept.
\begin{definition}[Coherent families of functions]\label{coherentfamiliesdef} A \textit{coherent family of functions} supported by an $\omega_1$-tower $\langle T_\alpha\rangle_{\alpha\in\omega_1\backslash \omega}$ is a family of functions $\langle f_\alpha \rangle_{\alpha\in\omega_1}$ such that:
\begin{enumerate}[label=$(\arabic*)$]
    \item $\forall \alpha\in \omega_1\backslash \omega\,(\,f_\alpha:T_\alpha\longrightarrow \alpha\,),$
\item $\forall \alpha,\beta\in \omega_1\backslash \omega\,(\,f_\alpha|_{T_\alpha\cap T_\beta}=^*f_\beta|_{T_\alpha\cap T_\beta}\,).$
\end{enumerate}
 Given such family, we define $L^\xi_\alpha$ as $f^{-1}_\alpha[\{\xi\}]$ for all $\xi\in \omega_1$ and $\alpha> \xi$. Additionally, we let $\mathcal{L}^{\xi}=\langle L^\xi_\alpha\rangle_{\alpha>\xi}$
 \end{definition}
 

Ilijas Farah constructed a Haudorff coherent family of functions supported by an $\omega_1$-tower by forcing it and then appealing to Keisler's completeness Theorem for $L^\omega(Q)$. Unlike Talayco's result, the proof idea behind the construction of Farah does not work for any $\omega_1$-tower. This is due to the nature of Keisler's Theorem. 

As an application of the concept of Luzin representations, we use Theorem \ref{luzinreptheorem} to generalize the results of Talayco, Todor\v{c}evi\'c, Morgan and Farah regarding the existence of \say{big gap cohomology groups}. It is worth noting that there is no  analogous to the $\aleph_0$ gap theorem for aribrary $*$-lower semi-lattices.


Therefore, we can not argue in the same way as Todor\v{c}evi\'c  in order to conclude that the gap cohomology group has always cardinality $2^{\omega_1}$.
\begin{theorem}\label{hausdorffcoherenttheorem}Let $(X,<,\wedge)$ be an $\omega_1$-like lower semi-lattice. Then there is a $*$-lower semi-lattice $\mathcal{T}$ isomorphic to $X$ with $|G(\mathcal{T})|=2^{\omega_1}.$
\begin{proof}Consider $X\times 2$ with the order given by $(x,i)<(y,j)$ if and only if $x<y$ and $i=j$. It is easy to see that $X\times 2$ is also $\omega_1$-like. In virtue of Theorem \ref{luzinreptheorem} we can take $\mathcal{T'}=\langle T'_{(x,i)}\rangle_{(x,i)\in X\times 2}$ and $\mathcal{A}=\langle A_{(x,i)}\rangle_{(x,i)\in X\times 2}$ so that $(\mathcal{T}',\mathcal{A})$ is an almost disjoint representation of $X\times 2$. For any $x\in X$ let $T_x=T'_{(x,0)}\cup T'_{(x,1)}. $ It is straightforward that the following properties hold for any $x,y \in X$:
\begin{enumerate}[label=$(\alph*)$]
\item $A_{(x,0)}\cup A_{(x,1)}\subseteq T_x$.

\item If $y\not\leq x$ then $A_{(y,0)}\cup A_{(y,1)}\subseteq^*T_y\backslash T_x$. In other words, $(A_{(y,0)}\cup A_{(y,1)})\cap T_x=^*\emptyset$.
\item $T_x\cap T_y=^*T_{x\wedge y}.$

\end{enumerate}
In particular, properties (b) and (c) imply that $\mathcal{T}=\langle T_x\rangle_{x\in X}$ is a $*$-lower semi-lattice isomorphic to $X$. We claim that $|G(\mathcal{T})|=2^{\omega_1}$. Trivially $|G(\mathcal{T})|\leq 2^{\omega_1}$, so we will only prove the other inequality. For this, let $S\in \mathscr{P}(X)$. . We will build recursively (using that $X$ is well-founded) a coherent subsystem $g_S:\mathcal{T}\longrightarrow \mathscr{P}(\omega)$ such that $A_{(x,0)}\subseteq g_S(T_x)$ for any $x\in X$ and:\\
\begin{center}\begin{minipage}{6cm} \begin{center} \textbf{(A)}\end{center} If $x\in S$, then $A_{(x,1)}\cap g_S(T_x)=^*\emptyset.$
\end{minipage}\hspace{2.5cm} \begin{minipage}{6cm}\begin{center} \textbf{(B)}\end{center} If $x\not\in S$, then $A_{(x,1)}\subseteq g_S(T_x)$.
\end{minipage}

\end{center}
Suppose that $y\in X$ and we have defined $g_S(T_x)$ for any $x<y$. By means of Lemma \ref{lemmacoherentsubsystempregap} we know that $\mathcal{G}(\mathcal{T}|_y,g_S|_{\mathcal{T}|_{y}})$ is pregap where $\mathcal{T}|_y=\langle T_x\rangle _{x<y}$. As there are no countable pregaps and $|(-\infty,y)|\leq \omega$, we conclude that there is $C\in \mathscr{P}(\omega)$ separating it.  Since $g_S(T_x)\subseteq T_x\subseteq^*T_y$ for any $x<y$, we may assume without loss of generality that $C\subseteq T_y$. Note that $C\cap T_x=^*g_S(T_x)$ for any $x<y$. We now define $g_S(T_y)$ by cases. If $y\in S$ define $g_S(T_y)$ as $(C\cup A_{(y,0)})\backslash A_{(y,1)}$. Otherwise define $g_S(T_y)$ as $C\cup A_{(y,0)}\cup A_{(y,1)}$. Since both $A_{(y,0)}$ and $A_{(y,1)}$ are almost disjoint with $T_x$ for all $x<y$ due to the point (b), it follows that $g_S(T_y)\cap T_x=^* C\cap T_x=^*g_S(T_x)$ for any such $x$. This finishes the recursion.

Now consider $\mathcal{S}\subseteq [X]^{\omega_1}$  a family of cardinality $2^{\omega_1}$ so that $S\Delta S'$ is uncountable for any two distinct $S,S'\in \mathcal{S}$. The key fact needed to finish the proof is that if $x\in S\Delta S'$ then $A_{(x,1)}\subseteq g_S\cdot g_{S'}(T_x)$ and $A_{(x,0)}\subseteq T_x\backslash (g_S\cdot g_{S'}(T_x))$.  In this way, any separation of the pregap  $\mathcal{G}(\mathcal{T},g_S\cdot g_{S'})$ would also separate the pregap $(A_{(x,1)},A_{(x,0)})_{x\in S\Delta S'}$ which is impossible since $\mathcal{A}$ is an inseparable family and $S\Delta S'$ is uncountable. This shows that $g_S$ and $g_{S'}$ are not cohomologous. Since $|S|=2^{\omega_1}$, then $|G(\mathcal{T})|=2^{\omega_1}$.
\end{proof}
\end{theorem}


